Human-Collective Collaborative Site Selection

Robotic collectives are large groups (at least 50) of locally sensing and communicating robots that encompass characteristics of swarms and colonies, whose emergent behaviors accomplish complex tasks. Future human-collective teams will extend the ability of operators to monitor, respond, and make decisions in disaster response, search and rescue, and environmental monitoring problems. This manuscript evaluates two collective best-of-n decision models for enabling collectives to identify and choose the highest valued target from a finite set of n targets. Two challenges impede the future use of human-collective shared decisions: 1) environmental bias reduces collective decision accuracy when poorer targets are easier to evaluate than higher quality targets, and 2) little is understood about shared human-collective decision making interaction strategies. The two evaluated collective best-of-n models include an existing insect colony decision model and an extended bias-reducing model that attempts to reduce environmental bias in order to improve accuracy. Collectives using these two strategies are compared independently and as members of human-collective teams. Independently, the extended model is slower than the original model, but the extended algorithm is 57% more accurate in decisions where the optimal option is more difficult to evaluate. Human-collective teams using the bias-reducing model require less operator influence and achieve 25% higher accuracy with difficult decisions, than the human-collective teams using the original model. Further, a novel human-collective interaction strategy enables operators to adjust collective autonomy while making multiple simultaneous decisions.

==> HCI_ECAS_4_Detailed_Situation.tex <==
Two experiments were conducted in order to test the influence of the different best-of-$n$ strategies (hypothesis $H_{1}$), the influence of the human operator on the decision process (hypothesis $H_{2}$), and the effectiveness of the collective visualization strategy used (hypothesis $H_{3}$).  Both experiments involved four  simulated robotic collectives that were required to make targeting decisions within an approximately $2$ km$^{2}$ environment.  Each collective had $200$ simulated Unmanned Aerial Vehicles (UAVs) that were limited to a $500$m exploration radius from the collectives' central decision making hubs.  Simulated robots behaved according to the models described in Section \ref{sec:CAS_Model}, which enabled each collective to perform explicit action selection within its coverage area.

The first experiment compared the performance of the two collective decision making models described in Section \ref{sec:CAS_Model} independent of a human operator.  Each of the four collectives completed a series of targeting selection decisions.  Each decision required the collective to select the highest valued target within its $500$m search range, move its decision making hub to the chosen target, and initiate the collective's next target selection decision.  Each target represented a location of interest that was assigned a value at the start of the scenario and remained invisible until at least two collective individuals discovered and favored the target and returned to the decision making hub.  Individual collective entities assessed a target's value, with a $10$\% error, when the individuals were within sensory range of the target.  After a collective selected a target and subsequently occupied the new location, the target was removed from the map, was no longer able to be discovered, and was replaced by a representation of the collective hub.  Collectives were capable of finding, evaluating, and occupying any target that was within their respective search ranges, which enabled multiple collectives to consider the same target during a decision.  After a collective moved, its next decision included all targets within range from the collective's new location.  

The second experiment evaluated human-collective teams.  Interactions between the individual collective entities and between the collective and the human operator were restricted to the collectives' decision making hubs.  The human operator was assumed to have access to intermittent satellite imagery (simulated using the Google API) and relied on communication with collective individuals within the collectives' decision making hubs. The operator was instructed to ensure that each collective chose the highest valued target every decision.  The operator monitored the collectives and issued requests to each collective as needed during the decision process.  Additionally, the  operator was instructed to prevent multiple collectives from choosing and occupying the same target site. Rarely ($0.6$\% of all decisions), two collectives did move to the same location.  The simulator accounted for this occurrence by automatically returning the second collective to reach the target to the collective's previous position, where it initiated a new target selection decision.    

Both experiments assumed a larger set of individual robot capabilities than those typically used in collective best-of-$n$ decision studies (e.g., \cite{ParkerZhang2009:CDMBestOfNProblem,Valentini2014:WeightedVoterModel,ReinaValentini:DesignPattern2015}).  Simple ground platforms, such as Kilobots \cite{kilobot} and e-Puck robots \cite{mondada_e-puck_2009} have been optimized for laboratory research. Both types of robots operate for long periods of time between battery charges (e.g., 2 hours for the e-Puck and several hours for the Kilobot) and are capable of short range ($<25$cm) peer to peer communication.  Each capability is central to many biologically-inspired collective decision making strategies (e.g.,  \cite{ParkerZhang2009:CDMBestOfNProblem,Valentini2014:WeightedVoterModel,ReinaValentini:DesignPattern2015,haque2016}), but are difficult to recreate in UAV collectives.  UAV peer-to-peer communication is complicated by the UAVs' high mobility \cite{FANET_Challenges,FSO_Majumdar2015}.   Many commercial rotor wing UAVs are capable of speeds of $60$km/h, but have limited flight times of approximately $25$ minutes (e.g., \cite{UAVCompare}). Despite these challenges, the simulated agents were assumed to have emergent capabilities and moved at $60$km/h for at least an hour of flight time and communicated via $30$m peer-to-peer transmissions (e.g., optical transmissions \cite{FSO_Alignment}).  A simplifying assumption was that robots moved at constant speed, which is similar to prior research \cite{cody_quorum_2017,ReinaValentini:DesignPattern2015}, but notably deviates from practical UAV movement.
